Nonparametric Embeddings of Sparse High-Order Interaction Events

High-order interaction events are common in real-world applications. Learning embeddings that encode the complex relationships of the participants from these events is of great importance in knowledge mining and predictive tasks. Despite the success of existing approaches, e.g. Poisson tensor factorization, they ignore the sparse structure underlying the data, namely the occurred interactions are far less than the possible interactions among all the participants. In this paper, we propose Nonparametric Embeddings of Sparse High-order interaction events (NESH). We hybridize a sparse hypergraph (tensor) process and a matrix Gaussian process to capture both the asymptotic structural sparsity within the interactions and nonlinear temporal relationships between the participants. We prove strong asymptotic bounds (including both a lower and an upper bound) of the sparsity ratio, which reveals the asymptotic properties of the sampled structure. We use batch-normalization, stick-breaking construction, and sparse variational GP approximations to develop an efficient, scalable model inference algorithm. We demonstrate the advantage of our approach in several real-world applications.

==> related.tex <==
\section{Related Work}
%interactions and tensor factorization & HPs
It is natural to represent high-order interactions by multidimensional arrays or tensors. Tensor factorization is the fundamental framework for tensor analysis. Classical tensor factorization approaches  include CP~\citep{Harshman70parafac}  and Tucker~\citep{Tucker66} decomposition, based on which numerous other methods have been proposed:~\citep{Chu09ptucker,kang2012gigatensor,YangDunson13Tensor,choi2014dfacto,du2018probabilistic,fang2021bayesian}, to name a  few. Recently, nonparametric and/or neural network  factorization models~\citep{zhe2015scalable,zhe2016distributed,zhe2016dintucker,liu2018neuralcp,pan2020streaming,tillinghast2020probabilistic,fang2021streaming,tillinghast2021nonparametric} were developed to estimate nonlinear relationships in data, and have shown advantages over popular multilinear methods in prediction accuracy. When dealing with temporal information, existing methods mainly use homogeneous Poisson processes and decompose the event counts~\citep{chi2012tensors,HaPlKo15,Hu2015CountTensor}. More advanced approaches further partition the time stamps into different steps, and perform count factorization across the time steps~\citep{xiong2010temporal, schein2015bayesian,Schein:2016:BPT:3045390.3045686,schein2019poisson}. Recently, \citet{zhe2018stochastic} used Hawkes processes to estimate the local triggering effects between the events, and modeled the triggering strength with a kernel of the embeddings of the interactions. \citet{pan2020scalable} modeled the time decay as another kernel of the embeddings, and developed scalable inference for long event sequences. \citet{wang2020self} proposed a non-Hawkes, non-Poisson process to estimate the triggering and inhibition effects between the events. All these are temporal point processes that focus on rate modeling, and are different from the PPPs (with mean measure) in \ours to sample sparse interaction structures. 
\citet{lloyd2015variational} proposed GP modulated Poisson processes and also used the square link to ensure a positive rate function.  However, the work is purely about event modeling and does not learn any embedding. With the SE kernel, it derives an analytical form of ELBO. However, since our model includes the embedding (log sociabilities) in the GP prior, the ELBO is analytically intractable, and we use the reparameterization trick to conduct stochastic optimization. Recently, \citet{pan2021self} proposed a self-adaptable point process for event modeling, which can estimate both the triggering and inhibition effects within the events. More important, they construct a GP based component to enable a nonparametric estimate of the time decays of these effects. Their point process is not a Poisson process any more. 

%sparse structures 
Our hyper-graph prior is inherited from the sparse tensor process in~\citep{tillinghast2021nonparametric}, which can be viewed as a multi-dimensional extension of the pioneer work of \citet{caron2014sparse,caron2017sparse}, who first  used completely random measures (CRMs)~\citep{kingman1967completely,kingman1992poisson,lijoi2010models}, such as Gamma processes (\gaps)~\citep{hougaard1986survival}, to generate sparse random graphs. \cmt{\citet{williamson2016nonparametric} considered the case of  Gamma processes~\citep{hougaard1986survival,brix1999generalized}, and used the normalized version, \ie Dirichlet processes~\citep{ferguson1973bayesian}, to develop models for link prediction.} However, these prior works only show the asymptotic sparse guarantee (\ie the sparsity ratio converges to zero at the limit), yet not giving any convergence rate estimate for popular \gaps that are convenient for  inference and computation.  Our work fills this gap by giving strong asymptotic bounds about the sparsity, including both a lower and upper bound, which can reveal more refined insight about these sparse priors. Furthermore, we couple the sparse  prior with matrix GPs  to jointly sample the interactions (\ie hyperedges) and their event sequences. In this way, the embeddings can assimilate both the sparse structural information underlying the present interactions and the hidden temporal relationship of the participants. 

\cmt{
In spite of the success of the existing models for interaction events, they overlook the sparse nature of the present interactions (against all possible interactions between the participants), and hence miss important structural information. To overcome this limitation, we view the participants of the interactions events as the nodes in a hypergraph, and their interactions as hyperedges. The event sequences are attached on the edges. We propose a stochastic process to sample the hypergraphs, with the guarantee of asymptotic sparsity. In the modeling of ordinary graphs,  \citet{caron2014sparse,caron2017sparse} first  used completely random measures (CRMs)~\citep{kingman1967completely,kingman1992poisson,lijoi2010models} to generate sparse random graphs. \citet{williamson2016nonparametric} considered the case of  Gamma processes~\citep{hougaard1986survival,brix1999generalized}, and used the normalized version, \ie Dirichlet processes~\citep{ferguson1973bayesian}, to develop models for link prediction. Our model can be viewed as an extension of these seminal works  for hypergraphs. Furthermore, we couple our stochastic hypergraph process with matrix Gaussian process  to jointly sample the interactions (\ie hyperedges) and their event sequences. In this way, the embeddings can assimilate both the sparse structural information underlying the present interactions and the hidden temporal relationships between the participant nodes. For sparse random graph generation,  \citet{crane2015framework,cai2016edge}  also proposed edge-exchange models; see thorough discussions in \citep{crane2018edge}. 
}
